FlowBench: A Large Scale Benchmark for Flow Simulation over Complex Geometries

Simulating fluid flow around arbitrary shapes is key to solving various engineering problems. However, simulating flow physics across complex geometries remains numerically challenging and computationally resource-intensive, particularly when using conventional PDE solvers. Machine learning methods offer attractive opportunities to create fast and adaptable PDE solvers. However, benchmark datasets to measure the performance of such methods are scarce, especially for flow physics across complex geometries. We introduce FlowBench, a dataset for neural simulators with over 10K samples, which is currently larger than any publicly available flow physics dataset. FlowBench contains flow simulation data across complex geometries (\textit{parametric vs. non-parametric}), spanning a range of flow conditions (\textit{Reynolds number and Grashoff number}), capturing a diverse array of flow phenomena (\textit{steady vs. transient; forced vs. free convection}), and for both 2D and 3D. FlowBench contains over 10K data samples, with each sample the outcome of a fully resolved, direct numerical simulation using a well-validated simulator framework designed for modeling transport phenomena in complex geometries. For each sample, we include velocity, pressure, and temperature field data at 3 different resolutions and several summary statistics features of engineering relevance (such as coefficients of lift and drag, and Nusselt numbers). %Additionally, we include masks and signed distance fields for each shape. We envision that FlowBench will enable evaluating the interplay between complex geometry, coupled flow phenomena, and data sufficiency on the performance of current, and future, neural PDE solvers. We enumerate several evaluation metrics to help rank order the performance of neural PDE solvers. We benchmark the performance of several baseline methods including FNO, CNO, WNO, and DeepONet.

==> Figures/chunking_alg.tex <==
\begin{algorithm}
\caption{Pair Creation}
\begin{algorithmic}[1]
\Procedure{Pair Creation}{$LayerA,LayerB,maxLength$}
    \State $start_i,start_j \gets 0,0$
    \State $end_i \gets maxLength$
    \State $pairs \gets List()$
    \While{$start_i <= \textbf{length}(LayerA)$}
        \State $end_j \gets start_j+1$
        \State $found \gets False$
        \While{$\neg found$ and $(end_j-start_j)\leq maxLength$}
            \If{$representation(LayerA[end_i])= representation(LayerB[end_j])$}
                \State $found \gets True$
            \EndIf
            \State $end_j = end_j + 1$
        \EndWhile
        \If{$found$} \Comment{Add matching pair of chunks to dataset}
            \State $chunk_a \gets LayerA[start_i:end_i]$
            \State $chunk_b \gets LayerB[start_j:end_j]$
            \State $pairs.append((chunk_a,chunk_b))$
        \Else 
            \State $end_i = end_i-1$ \Comment{Could not find a line matching line $end_i$, try a smaller chunk}
        \EndIf
    \EndWhile
    \State \Return $LayerA, FlippedB$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> Figures/contour_flip_alg.tex <==
\begin{algorithm}
\caption{Contour Flipping}
\begin{algorithmic}[1]
\Procedure{ContourFlip}{$LayerA,LayerB$}
    \State $ContoursA \gets ContourSplit(LayerA)$
    \State $ContoursB \gets ContourSplit(LayerB)$
    \State $Lookup \gets HashMap()$ \Comment{Create hash index of contours in Layer B}
    \For{$c \gets 1$ to \textbf{length}($ContoursB$)}
        \For{$i \gets 1$ to \textbf{length}($ContoursB[c]$)}
            \State $line_i \gets representation(ContoursB[c][i])$
            \If{$line_i \in Lookup$ and $Lookup[line_i]\neq i$}
                \State Delete $Lookup[line_i]$
            \Else 
                \State $Lookup[line_i] \gets c$
            \EndIf
        \EndFor
    \EndFor
    \State $Mapping \gets HashMap()$ \Comment{Find bijection between layers}
    \For{$c_A \gets 1$ to \textbf{length}($ContoursA$)}
        \For{$i \gets 1$ to \textbf{length}($ContoursA[c_A]$)}
            \State $line_i \gets representation(ContoursA[c_A][i])$
            \If{$line_i \in Lookup$}
                \State $ c_B \gets Lookup[line_i]$
                \State $Mapping[c_B] \gets c_A$
            \EndIf
        \EndFor
    \EndFor
    \State $FlippedB \gets Array[\textbf{length}(ContoursB[c_A])]$ 
    \For{$i \gets 1$ to \textbf{length}($ContoursB$)}
        \State $FlippedB[Mapping[c_i]] \gets ContoursB[i]$
    \EndFor
    \State \Return $LayerA, FlippedB$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> abstract_sub.tex <==
\begin{comment}


Simulating fluid flow around arbitrary shapes is key to various engineering problems. However, simulating flow physics across complex geometries remains numerically challenging and computationally resource-intensive. Machine learning methods can create fast, accurate, and robust solvers. There is a shortage of benchmark datasets to train and test such models, especially for flow physics across complex geometries. 

We introduce $\textbf{FlowBench}$, a benchmark for neural simulators with 10X more samples than any publicly available flow physics dataset. $\textbf{FlowBench}$ contains flow simulation data across complex geometries ($\textit{parametric vs. non-parametric}$), and spanning a range of flow conditions ($\textit{Reynolds number and Grashoff number}$), thus capturing a diverse array of flow phenomena ($\textit{steady vs. transient; forced vs. neutral vs. free convection}$) in both 2D and 3D. $\textbf{FlowBench}$ contains nearly 10,000 data samples, with each sample the outcome of a fully resolved, direct numerical simulation (DNS) performed using a well-validated simulator framework designed for modeling transport phenomena in complex geometries. For each sample, we include velocity, pressure, and temperature field data at 3 different resolutions and several summary statistics features of engineering relevance (like coefficients of lift and drag and Nusselt numbers). Additionally, we include masks and signed distance fields for each shape. 

$\textbf{FlowBench}$ is a comprehensive benchmark for evaluating the interplay between complex geometry, coupled flow phenomena, and data sufficiency on the performance of current, and next-gen neural PDE solvers. We enumerate several evaluation metrics to help rank order the performance of current (and future) neural PDE solvers. We test three baseline SciML models, viz. Fourier Neural Operators (FNO), Convolutional Neural Operators (CNO), and DeepONet. Our results suggest promising accuracy in learning the complex fluid dynamics around 2D and 3D objects using neural PDE solvers.

    

    
emails:
rtali@iastate.edu, Ronak Tali
arabeh@iastate.edu, Ali Rabeh
chenghau@iastate.edu, Cheng-Hau Yang
mehdish@iastate.edu, Mehdi Shadkhah
samundra@iastate.edu, Samundra Karki
au2216@nyu.edu, Abhisek Upadhyaya
snarayan@iastate.edu, Suriya Dhakshinamoorthy
marjansd@iastate.edu, Marjan Saadati
soumiks@iastate.edu, Soumik Sarkar
adarsh@iastate.edu, Adarsh Krishnamurthy
chinmay.h@nyu.edu, Chinmay Hegde
baditya@iastate.edu, Aditya Balu
baskarg@iastate.edu, Baskar Ganapathysubramanian 


\end{comment}
